Bifurcations of the polycycle "tears of the heart": multiple numerical invariants

"Tears of the heart" is a hyperbolic polycycle formed by three separatrix connections of two saddles. It is met in generic 3-parameter families of planar vector fields. In [arXiv:1506.06797], it was discovered that generically, the bifurcation of a vector field with "tears of the heart" is structurally unstable. The authors proved that the classification of such bifurcations has a numerical invariant. In this article, we study the bifurcations of "tears of the heart" in more detail, and find out that the classification of such bifurcation may have arbitrarily many numerical invariants.

==> Makefile <==
PDFLATEX=pdflatex -synctex=1
LUALATEX=lualatex -synctex=1

MAINFILE=tearsHeart
NOLUA=$(MAINFILE)-nolua
BIBFILES=$(shell grep addbibresource $(MAINFILE).tex | sed -e 's,^\\addbibresource{,,' -e 's,}$$,,')
BIBPATHS=$(shell kpsewhich $(BIBFILES))

SVG_FILES = $(shell git ls-files *.svg)
PDF_PICTURES = $(patsubst %.svg,%.pdf,$(SVG_FILES))

default: pdf update-ignore source.zip

pdf: $(NOLUA).pdf $(MAINFILE).pdf

.PHONY: pdf clean update-ignore default

%.bib.txt:
	ln -sv $$(kpsewhich $*.bib) $@

%.pdf: %.svg
	inkscape $< -D -A $@

clean:
	rm -f -v $(PDF_PICTURES)
	git clean -fx $(MAINFILE).* $(NOLUA).*

$(NOLUA).tex: $(MAINFILE).tex de-unicode.sed
	sed -f de-unicode.sed < $< > $@

$(NOLUA).bcf: $(NOLUA).tex $(PDF_PICTURES)
	$(PDFLATEX) $<

$(NOLUA).bbl: $(NOLUA).bcf
	biber $<
	sed -f de-unicode.sed -i $@

$(NOLUA).pdf: $(NOLUA).tex $(NOLUA).bbl $(PDF_PICTURES)
	$(PDFLATEX) $<
	$(PDFLATEX) $<

$(MAINFILE).tex.orig:
	ln -sv $(MAINFILE).tex $(MAINFILE).tex.orig

$(MAINFILE).bcf: $(MAINFILE).tex $(PDF_PICTURES)
	$(LUALATEX) $(MAINFILE)

$(MAINFILE).bbl: $(MAINFILE).bcf
	biber $<

$(MAINFILE).pdf: $(MAINFILE).tex $(MAINFILE).bbl $(PDF_PICTURES)
	$(LUALATEX) $<
	$(LUALATEX) $<

source.zip: $(subst .bib,.bib.txt,$(BIBFILES)) $(NOLUA).bbl $(MAINFILE).tex.orig $(NOLUA).tex $(PDF_PICTURES) Makefile
	zip -FS $@ $^

update-ignore:
	sed -e '/AUTO UPDATE/,$$d' -i .gitignore
	echo "# AUTO UPDATE" >> .gitignore
	for f in $(PDF_PICTURES); do echo $$f; done | sort >> .gitignore
	echo "$(NOLUA).*" >> .gitignore
	echo "$(MAINFILE).*" >> .gitignore
	echo "!$(MAINFILE).tex" >> .gitignore
	echo "source.zip" >> .gitignore
	echo "*.bib.txt" >> .gitignore

